Reduction of power grid fluctuations by communication between smart devices

The increase of electric demand and the progressive integration of renewable sources threatens the stability of the power grid. To solve this issue, several methods have been proposed to control the demand side instead of increasing the spinning reserve on the supply side. Here we focus on dynamic demand control (DDC), a method in which appliances can delay its scheduled operation if the electric frequency is outside a suitable range. We have recently shown that DDC effectively reduces small and medium-size frequency fluctuations but, due to the need of recovering pending tasks, the probability of large demand peaks, and hence large frequency fluctuations, may actually increase. Although these events are very rare they can potentially trigger a failure of the system and therefore strategies to avoid them have to be addressed. In this work, we introduce a new method including communication among DDC devices belonging to a given group, such that they can coordinate opposite actions to keep the group demand more stable. We show that for this method the amount of pending tasks decreases by a factor 10 while large frequency fluctuations are significantly reduced or even completely avoided.

==> interaction.tex <==
@ARTICLE{Figueredo:2009dg,
   author = {Figueredo, A. J. and Wolf, P. S.~A.},
   title = {Assortative pairing and life history strategy - a cross-cultural study.},
   journal = {Human Nature},
   volume = {20},
   pages = {317-330},
   year = {2009}
}

@ARTICLE{Tchawou1,
   author = {Tchawou Tchuisseu, E. B. and Gomila, D. and Brunner, D. and Colet, P},
   title = {Effects of dynamic-demand-control appliances on the power grid frequency},
   journal = {Phys. Rev. E},
   volume = 96,
   pages = 022302,
   year = 2017
}
@book{Murray_Springer_2002,
   author =   {J. D. Murray},
   title =        {Mathematical Biology (vols. 1 and 2)},
   publisher = {Springer},
   edition = {3rd},
   address = {New York},
   year = {2002}
 }    

@phdthesis{hamon2012,
   author = {Hamon, C}, 
   title = {On frequency control schemes in power systems with large amounts of wind power},
   school = {KTH Royal Institute of Technology},
   year = 2012
}
 

@ARTICLE{Rebours2007,
author={Y. G. Rebours and D. S. Kirschen and M. Trotignon and S. Rossignol},
journal={IEEE Transactions on Power Systems},
title={A Survey of Frequency and Voltage Control Ancillary Services mdash;Part I: Technical Features},
year={2007},
volume={22},
number={1},
pages={350-357},
keywords={frequency control;power system control;power system economics;voltage control;active power reserves;economic features;frequency-voltage control ancillary services;Automatic generation control;Europe;Frequency control;Legged locomotion;Power generation;Power generation economics;Power system control;Power system economics;Power systems;Voltage control;Ancillary services;frequency control;reactive power;spinning reserve;system services;voltage control},
doi={10.1109/TPWRS.2006.888963},
ISSN={0885-8950},
month={Feb},}
 
@ARTICLE{Short07,
author={J. A. Short and D. G. Infield and L. L. Freris},
journal={IEEE Transactions on Power Systems},
title={Stabilization of Grid Frequency Through Dynamic Demand Control},
year={2007},
volume={22},
number={3},
pages={1284-1293},
keywords={demand side management;frequency control;power generation control;power generation faults;power system stability;refrigerators;consumer appliances;dynamic demand control;electricity networks;grid frequency stabilization;refrigerators;supply quality maintenance;Computerized monitoring;Frequency;Grid computing;Home appliances;Power generation;Power system dynamics;Power system modeling;Stability;Switches;Wind energy generation;Dynamic demand;demand-side management;dynamic demand control;frequency control;integration of renewable power generation;intelligent load;power system stability;refrigerators},
doi={10.1109/TPWRS.2007.901489},
ISSN={0885-8950},
month={Aug},}

@article{Dehghanpour,
title = {Electrical demand side contribution to frequency control in power systems: a review on technical aspects},
journal = {Renewable and Sustainable Energy Reviews},
volume = 41,
pages = {1267 - 1276},
year = 2015,
issn = {1364-0321},
doi = {https://doi.org/10.1016/j.rser.2014.09.015},
url = {http://www.sciencedirect.com/science/article/pii/S1364032114007886},
author = {Kaveh Dehghanpour and Saeed Afsharnia},
keywords = {Frequency control, Demand response, Centralized and decentralized control, Synchronization}
}



@article{haider2016review,
title = {A review of residential demand response of smart grid},
journal = {Renewable and Sustainable Energy Reviews},
volume = 59,
pages = {166 - 178},
year = 2016,
issn = {1364-0321},
doi = {https://doi.org/10.1016/j.rser.2016.01.016},
url = {http://www.sciencedirect.com/science/article/pii/S1364032116000447},
author = {Haider Tarish Haider and Ong Hang See and Wilfried Elmenreich},
keywords = {Smart grids, Residential demand response, Load scheduling, Information and communication technologies, Internet of Things}
}

@article{alberini2011, 
title = {Response of residential electricity demand to price: The effect of measurement error},
journal = {Energy Economics"},
volume = 33,
number = 5,
pages = {889 - 895},
year = 2011,
issn = {0140-9883},
doi = {https://doi.org/10.1016/j.eneco.2011.03.009},
url = {http://www.sciencedirect.com/science/article/pii/S0140988311000776},
author = {Anna Alberini and Massimo Filippini},
keywords = {Residential electricity, Gas demand, US states, Panel data, Dynamic panel data models, Partial adjustment model}
}

@article{esther2016,
title = {A survey on residential Demand Side Management architecture, approaches, optimization models and methods},
journal = {Renewable and Sustainable Energy Reviews},
volume = {59},
pages = {342 - 351},
year = {2016},
issn = {1364-0321},
doi = {https://doi.org/10.1016/j.rser.2015.12.282},
url = {http://www.sciencedirect.com/science/article/pii/S1364032115016652},
author = {B. Priya Esther and K. Sathish Kumar},
keywords = {Demand Side Management (DSM), Demand response (DR), Home Energy Management (HEM)}
}

@article{Albadi2008,
title = {A summary of demand response in electricity markets},
journal = {Electric Power Systems Research},
volume = {78},
number = {11},
pages = {1989 - 1996},
year = {2008},
issn = {0378-7796},
doi = {https://doi.org/10.1016/j.epsr.2008.04.002},
url = {http://www.sciencedirect.com/science/article/pii/S0378779608001272},
author = {M.H. Albadi and E.F. El-Saadany},
keywords = {Demand response, Price elasticity, Real time pricing, Electricity markets}
}

@techreport {US_DEPARTMENT,
title = {Benefits of Demand Response in Electricity Markets and Recommendations for Achieving Them - A Report to the United States Congress Pursant to Section 1252 of the Energy Policy Act of 2005},
year = {2006},
month = {02/2006},
pages = {122},
institution = {U.S. Department of Energy},
keywords = {electricity markets and policy group, energy analysis and environmental impacts department},
author = {U.S. Department of Energy},
howpublished = {available online: http://eetd.lbl.gov.}
}

@INPROCEEDINGS{Albadi2007,
author={M. H. Albadi and E. F. El-Saadany},
booktitle={2007 IEEE Power Engineering Society General Meeting},
title={Demand Response in Electricity Markets: An Overview},
year={2007},
volume={},
number={},
pages={1-5},
keywords={demand side management;power markets;demand response;electricity markets;incentive based programs;market based programs;price based programs;price elasticity;real time pricing;Costs;Distributed power generation;Electricity supply industry;Energy consumption;Load management;Potential well;Pricing;Reliability;Thermostats;Timing;Demand Response;Incentive based programs;Market based programs;Price elasticity;Price-based programs;Real time pricing},
doi={10.1109/PES.2007.385728},
ISSN={1932-5517},
month={June},}

@INPROCEEDINGS{Lu2006,
author={Ning Lu and T. Nguyen},
booktitle={2005/2006 IEEE/PES Transmission and Distribution Conference and Exhibition},
title={Grid Friendly Appliances - Load-side Solution for Congestion Management},
year={2006},
volume={},
number={},
pages={1269-1273},
keywords={HVAC;demand side management;domestic appliances;power consumption;power markets;pricing;HVAC load;competitive electricity market;congestion management;congestion price;frequency signals detection;grid friendly appliances;load reduction;load-side solution;power consumption;power grid;price detection;residential house ventilation and air conditioning load;sensor;thermostat;transmission lines;voltage detection;Air conditioning;Electricity supply industry;Energy management;Frequency;Home appliances;Power transmission lines;Thermal sensors;Thermostats;Ventilation;Voltage control},
doi={10.1109/TDC.2006.1668693},
ISSN={2160-8555},
month={May},}

@ARTICLE{Schweppe,
author={F. C. Schweppe and R. D. Tabors and J. L. Kirtley and H. R. Outhred and F. H. Pickel and A. J. Cox},
journal={IEEE Transactions on Power Apparatus and Systems},
title={Homeostatic Utility Control},
year={1980},
volume={PAS-99},
number={3},
pages={1151-1163},
keywords={Automatic control;Automatic generation control;Control systems;Costs;Dispersion;Distributed power generation;Home automation;Power system control;Power systems;Storage automation},
doi={10.1109/TPAS.1980.319745},
ISSN={0018-9510},
month={May},}

@INPROCEEDINGS{Lasseter1,
author={R. H. Lasseter},
booktitle={2002 IEEE Power Engineering Society Winter Meeting. Conference Proceedings (Cat. No.02CH37309)},
title={MicroGrids},
year={2002},
volume={1},
number={},
pages={305-308 vol.1},
keywords={distribution networks;invertors;power generation control;power generation protection;reactive power control;voltage control;MicroGrid;dispatchable load;feeder losses reduction;frequency droop;loads cluster;local voltages support;microsource controller;microsources;microturbines;power electronics;power sharing;protection;reactive power control;real power control;reliability enhancement;single controllable system;transmission system;uninterruptible power supply;voltage regulation;voltage sag correction;voltage source inverter;waste heat;Communication system control;Control systems;Fuel cells;Inverters;Load flow;Power electronics;Power system protection;Power system reliability;Temperature control;Voltage fluctuations},
doi={10.1109/PESW.2002.985003},
ISSN={},
month={},}

@INPROCEEDINGS{Lasseter2,
author={R. H. Lasseter},
booktitle={2007 IEEE International Conference on System of Systems Engineering},
title={Certs Microgrid},
year={2007},
volume={},
number={},
pages={1-5},
keywords={distributed power generation;power distribution reliability;power supply quality;uninterruptible power supplies;CERTS mlcrogrid;UPS services;distributed generators;electric reliability technology solutions;power quality;Distributed control;Distributed power generation;Frequency;Peer to peer computing;Power system protection;Switches;Uninterruptible power systems;Voltage;Waste heat;Water heating;CHP;UPS;distributed generation;intentional islanding;inverters;microgrid;power vs. frequency droop;voltage droop},
doi={10.1109/SYSOSE.2007.4304248},
ISSN={},
month={April},}

@article{Lemoine,
  author={D M Lemoine and D M Kammen and A E Farrell},
  title={An innovation and policy agenda for commercially competitive plug-in hybrid electric vehicles},
  journal={Environmental Research Letters},
  volume={3},
  number={1},
  pages={014003},
  url={http://stacks.iop.org/1748-9326/3/i=1/a=014003},
  year={2008},
}

@ARTICLE{Doherty,
author={R. Doherty and M. O'Malley},
journal={IEEE Transactions on Power Systems},
title={A new approach to quantify reserve demand in systems with significant installed wind capacity},
year={2005},
volume={20},
number={2},
pages={587-595},
keywords={load forecasting;power generation faults;power generation reliability;power system security;wind power plants;Ireland electricity system;generator outage rates;power forecast;power generation faults;power generation reliability;power generation security;power penetration;wind power capacity;Load forecasting;Power generation;Power measurement;Power system modeling;Power system reliability;Wind energy;Wind energy generation;Wind farms;Wind forecasting;Wind power generation;Forecasting;power generation faults;power system security;wind power generation},
doi={10.1109/TPWRS.2005.846206},
ISSN={0885-8950},
month={May},}

@INPROCEEDINGS{Nehrir,
author={M. H. Nehrir and B. J. LaMeres and V. Gerez},
booktitle={IEEE Power Engineering Society. 1999 Winter Meeting (Cat. No.99CH36233)},
title={A customer-interactive electric water heater demand-side management strategy using fuzzy logic},
year={1999},
volume={1},
number={},
pages={433-436 vol.1},
keywords={control system analysis;control system synthesis;demand side management;electric heating;fuzzy control;load distribution;power system control;control design;control simulation;customer-interactive electric water heater DSM;distribution area water heaters;distribution demand profile levelling;electricity demand;fuzzy controller;fuzzy logic-based DSM;peak load shifting;power demand profile;Energy consumption;Energy management;Fuzzy control;Fuzzy logic;Power demand;Resistance heating;Temperature control;Voltage control;Water heating;Water storage},
doi={10.1109/PESW.1999.747494},
ISSN={},
month={Jan},}

@ARTICLE{Brooks,
author={Alec Brooks and Ed Lu and Dan Reicher and Charles Spirakis and Bill Weihl},
journal={IEEE Power and Energy Magazine},
title = {Demand Dispatch - Using Real-Time Control of Demand to help Balance Generation and Load},
year={2010},
volume={8},
number={3},
pages={20-29},
keywords={demand side management;power generation dispatch;power grids;demand dispatch;electric power grid;plug-in electric vehicles;smart charging;Aggregates;Bandwidth;Communication system control;Communications technology;Delay;IP networks;Load management;Mesh generation;Power generation;Protocols},
doi={10.1109/MPE.2010.936349},
ISSN={1540-7977},
month={May},}

@INPROCEEDINGS{Shively,
author={D. Shively and J. Gardner and T. Haynes and J. Ferguson},
booktitle={2008 IEEE Energy 2030 Conference},
title={Energy Storage Methods for Renewable Energy Integration and Grid Support},
year={2008},
volume={},
number={},
pages={1-6},
keywords={compressed air energy storage;pumped-storage power stations;solar power;wind power;compressed air energy storage;fossil fuels;grid support;pumped-storage power stations;renewable energy integration;solar installations;solar power;wind farms;wind power;Combustion;Energy storage;Fluctuations;Pumps;Renewable energy resources;Solar power generation;Turbines;Wind energy;Wind energy generation;Wind farms},
doi={10.1109/ENERGY.2008.4781002},
ISSN={},
month={Nov},}

@INPROCEEDINGS{Takagi,
author={M. Takagi and K. Yamaji and H. Yamamoto},
booktitle={2009 IEEE Vehicle Power and Propulsion Conference},
title={Power system stabilization by charging power management of Plug-in Hybrid Electric Vehicles with LFC signal},
year={2009},
volume={},
number={},
pages={822-826},
keywords={hybrid electric vehicles;power system stability;area control error;charging power management;load frequency control;plug-in hybrid electric vehicles;power system stabilization;wind power generation;Energy management;Frequency control;Frequency conversion;Hybrid electric vehicles;Hybrid power systems;Power control;Power system interconnection;Power system management;Power system modeling;Power system restoration;area control error;charging power contro;load frequency control;plug-in hybrid electric vehicle;tie-linel;wind power generation},
doi={10.1109/VPPC.2009.5289763},
ISSN={1938-8756},
month={Sept},}

@ARTICLE{Molderink,
author={A. Molderink and V. Bakker and M. G. C. Bosman and J. L. Hurink and G. J. M. Smit},
journal={IEEE Transactions on Smart Grid},
title={Management and Control of Domestic Smart Grid Technology},
year={2010},
volume={1},
number={2},
pages={109-119},
keywords={demand side management;distributed power generation;domestic appliances;electricity supply industry;power consumption;power distribution control;power generation control;smart power grids;demand and supply;demand side load management;distributed energy generation;distributed energy storage;domestic appliance planning;domestic smart grid control;domestic smart grid management;energy consumption;energy efficient electricity supply chain;energy production;energy stream optimization;greenhouse effect reduction;grid stability;real-time domestic appliance control;virtual power plant;Distributed control;Energy consumption;Energy efficiency;Energy storage;Load management;Optimized production technology;Smart grids;Stability;Supply chains;Technology management;Energy efficiency;microgeneration;microgrid;smart grid;virtual power plant},
doi={10.1109/TSG.2010.2055904},
ISSN={1949-3053},
month={Sept},}

@INPROCEEDINGS{Kosek,
author={A. M. Kosek and G. T. Costanzo and H. W. Bindner and O. Gehrke},
booktitle={2013 IEEE International Conference on Smart Energy Grid Engineering (SEGE)},
title={An overview of demand side management control schemes for buildings in smart grids},
year={2013},
volume={},
number={},
pages={1-9},
keywords={building management systems;decision support systems;demand side management;load regulation;power system control;power system management;power system stability;smart power grids;decision support system;demand side management control scheme;distributed energy resource;distribution network operation;energy production;failure handling;load control policy classification;load management;power system;renewable energy resource;smart building;smart power grid;stability;Buildings;Computer architecture;Control systems;Density estimation robust algorithm;Power systems;Production;Schedules},
doi={10.1109/SEGE.2013.6707934},
ISSN={},
month={Aug},}
   
@misc{Parliament,
   title = {Parliament of the {United Kingdom} electricity act}, 
   year = 1989,
   url = {https://www.legislation.gov.uk/ukpga/1989/29/contents},
}   

@book{Nick,
  title={Energy Science: Principles, Technologies, and Impacts},
  author={Andrews, J. and Jelley, N. and Jelley, N.A.},
  isbn={9780198755814},
  lccn={2016961067},
  url={https://books.google.es/books?id=RD0lDwAAQBAJ},
  year={2017},
  publisher={Oxford University Press}
}
   

@misc{National,
   title = {{UK National Grid Realtime}} 
   url={https://extranet.nationalgrid.com/RealTime}
}

@misc{hirst_2001, title={Responsive Load System}, author={Hirst, D}, year={2001}, month={Oct}}

@ARTICLE{Hirst,
author= {D. Hirst}, 
journal = {U.K. patent},
    title = {Responsive Load System},
    volume={},
    pages = {GB2361118},
    year = {2001},
    month={Oct},
}

@ARTICLE{Trevor,
author = {A.M. Trevor},
title = {Using Dishwashers to Provide Frequency Regulation Through Dynamic Demand}, 
journal = {Conference Papers/Science Symposium},
year = {2011},
}   

@ARTICLE{Hild,
author={S. Hild and S. Leavey and C. Gräf and B. Sorazu},
journal={IEEE Transactions on Smart Grid},
title={Smart Charging Technologies for Portable Electronic Devices},
year={2014},
volume={5},
number={1},
pages={328-336},
keywords={battery management systems;load regulation;mobile handsets;portable computers;power supply circuits;secondary cells;smart power grids;battery charge status;built-in energy storage;charging process;complex control routine;demand side control;electricity grid frequency;electricity grid stability;laptop computer;mobile phone;portable electronic device;short term power production fluctuations;smart charging technology;software implementation;tablet computer;Batteries;Electricity;Frequency control;Frequency measurement;Hardware;Microcontrollers;Portable computers;Demand side control;smart charging;smart grids},
doi={10.1109/TSG.2013.2281853},
ISSN={1949-3053},
month={Jan},}

@INPROCEEDINGS{Moghadam,
author={M. R. Vedady Moghadam and R. T. B. Ma and R. Zhang},
booktitle={2013 IEEE International Conference on Acoustics, Speech and Signal Processing},
title={Distributed frequency control via demand response in smart grids},
year={2013},
volume={},
number={},
pages={5233-5237},
keywords={automatic gain control;distributed control;frequency control;power system control;smart power grids;synchronisation;Ireland power system;automatic generation controllers;baseline hysteresis algorithm;demand response;distributed control algorithm;distributed demand response;distributed frequency control;frequency responsive demand control;generation side controllers;grid dependency;isochoronous governors;power grid reliability;power grid stability;power system frequency;randomized frequency monitoring;smart appliances;smart grids;synchronization problem;system frequency dynamics;Frequency control;Home appliances;Load management;Power demand;Power system dynamics;Power system stability;Time-frequency analysis;Smart grid;demand response;distributed algorithm;frequency control},
doi={10.1109/ICASSP.2013.6638661},
ISSN={1520-6149},
month={May},}

@ARTICLE{Moghadam2,
author={M. R. Vedady Moghadam and R. T. B. Ma and R. Zhang},
journal={IEEE Transactions on Smart Grid},
title={Distributed Frequency Control in Smart Grids via Randomized Demand Response},
year={2014},
volume={5},
number={6},
pages={2798-2809},
keywords={demand side management;distributed control;domestic appliances;frequency control;frequency stability;power consumption;power generation control;power system stability;randomised algorithms;smart power grids;distributed frequency control algorithm;frequency dynamics analysis;frequency oscillation problem;frequency recovery time;generation side controller;power consumption variation;power system frequency stabilisation;randomized demand response algorithm;smart appliances;smart power grid reliability;smart power grid stability;Frequency control;Home appliances;Load management;Power demand;Time-frequency analysis;Demand response;distributed frequency control;randomized algorithm;smart grids},
doi={10.1109/TSG.2014.2316913},
ISSN={1949-3053},
month={Nov},}

@ARTICLE{Luo,
author={Q. Luo and K. B. Ariyur and A. K. Mathur},
journal={IEEE Transactions on Smart Grid},
title={Will the Smart Grid Be Stable: Approaches for Supply-Demand Imbalances},
year={2014},
volume={5},
number={3},
pages={1361-1368},
keywords={demand side management;power markets;smart power grids;supply and demand;current deregulated market structure;current grid equipment;electric utilities;engineering analysis;real time energy management;real time pricing;smart grid;solar energy;supply demand imbalances;Buildings;Contracts;Electricity;Power generation;Production;Real-time systems;Solar radiation;Distributed generation;hedging;solar power},
doi={10.1109/TSG.2013.2272181},
ISSN={1949-3053},
month={May},}

@article{Escriva,
title = {Application of an energy management and control system to assess the potential of different control strategies in HVAC systems},
journal = {Energy and Buildings},
volume = {42},
number = {11},
pages = {2258 - 2267},
year = {2010},
issn = {0378-7788},
doi = {https://doi.org/10.1016/j.enbuild.2010.07.023},
url = {http://www.sciencedirect.com/science/article/pii/S0378778810002537},
author = {Guillermo Escriv\'a-Escriv\'a and Isidoro Segura-Heras and Manuel Alc\'azar-Ortega},
keywords = {Energy saving strategies, Energy management and control system, HVAC split system, Demand response}
}

@ARTICLE{Alvarez,
author={C. Alvarez and A. Gabaldon and A. Molina},
journal={IEEE Transactions on Power Systems},
title={Assessment and simulation of the responsive demand potential in end-user facilities: application to a university customer},
year={2004},
volume={19},
number={2},
pages={1223-1231},
keywords={demand side management;educational institutions;power consumption;power markets;ancillary service;demand side management program;electricity consumption;electricity market;end-user facilities;network constraints;responsive demand potential;university customer;voluntary demand participation program;Commercialization;Elasticity;Electricity supply industry;Energy consumption;Energy management;Energy storage;Home appliances;Packaging;Power engineering and energy;Power generation},
doi={10.1109/TPWRS.2004.825878},
ISSN={0885-8950},
month={May},}

@ARTICLE{Mohsenian,
author={A. H. Mohsenian-Rad and V. W. S. Wong and J. Jatskevich and R. Schober and A. Leon-Garcia},
journal={IEEE Transactions on Smart Grid},
title={Autonomous Demand-Side Management Based on Game-Theoretic Energy Consumption Scheduling for the Future Smart Grid},
year={2010},
volume={1},
number={3},
pages={320-331},
keywords={power consumption;power generation scheduling;smart power grids;Nash equilibrium;autonomous demand-side management;demand-side management programs;game-theoretic energy consumption scheduling;smart grid;Cost function;Distributed algorithms;Energy consumption;Game theory;Peak to average power ratio;Pricing;Smart grids;Demand-side management;distributed algorithms;energy consumption scheduling;energy pricing;game theory;market incentives;smart grid;smart meter},
doi={10.1109/TSG.2010.2089069},
ISSN={1949-3053},
month={Dec},}

@ARTICLE{Ruiz,
author={N. Ruiz and I. Cobelo and J. Oyarzabal},
journal={IEEE Transactions on Power Systems},
title={A Direct Load Control Model for Virtual Power Plant Management},
year={2009},
volume={24},
number={2},
pages={959-966},
keywords={domestic appliances;load regulation;optimal control;optimisation;power markets;power system management;thermostats;direct load control model;distributed energy resources;distributed generation;distribution networks;liberalized electricity markets;load reduction;optimal control;optimization algorithm;thermostatically controlled appliances;transmission networks;virtual power plant management;Density estimation robust algorithm;Distributed control;Electricity supply industry;Energy management;Energy resources;Load flow control;Load modeling;Optimal control;Power generation;Power system modeling;Air-conditioning;load management;optimal control},
doi={10.1109/TPWRS.2009.2016607},
ISSN={0885-8950},
month={May},}

@ARTICLE{Shi,
author={W. Shi and N. Li and X. Xie and C. C. Chu and R. Gadh},
journal={IEEE Journal on Selected Areas in Communications},
title={Optimal Residential Demand Response in Distribution Networks},
year={2014},
volume={32},
number={7},
pages={1441-1450},
keywords={demand side management;load flow;load shedding;power consumption;power distribution economics;supply and demand;IEEE test distribution system;distribution networks;electricity consumption;electricity shedding;electricity usage;load service entity;optimal demand schedule;optimal power flow;optimal residential demand response;power distribution network;residential DR parameters;supply and demand;supply-demand matching;Aggregates;Electricity;Home appliances;Load modeling;Power systems;Schedules;Simulation;Demand response (DR);distributed algorithms;distribution networks;optimal power flow (OPF);smart grid},
doi={10.1109/JSAC.2014.2332131},
ISSN={0733-8716},
month={July},}

@article{Shu, 
title={Demand response based on voluntary time-dependent pricing scheme}, 
volume={3}, DOI={10.1017/ATSIP.2014.10}, 
journal={APSIPA Transactions on Signal and Information Processing}, 
publisher={Cambridge University Press}, 
author={Shu, Haiyan and Yang, Wenxian and Chai, Chin Choy and Yu, Rongshan}, 
year={2014}, 
pages={e11}}

@ARTICLE{Qian,
author={L. P. Qian and Y. J. A. Zhang and J. Huang and Y. Wu},
journal={IEEE Journal on Selected Areas in Communications},
title={Demand Response Management via Real-Time Electricity Price Control in Smart Grids},
year={2013},
volume={31},
number={7},
pages={1268-1280},
keywords={demand forecasting;demand side management;energy consumption;iterative methods;optimisation;pricing;smart power grids;SAPC algorithm;demand response management;energy consumption;forecasted user reactions;iterative algorithm;message exchanges;nonconvex price optimization problem;quality-of-usage;real-time electricity price control;simulated-annealing-based price control;smart grids;two-stage optimization problem;Demand response management;Non-convex optimization;Payoff maximization;Profit maximization;Real-time pricing},
doi={10.1109/JSAC.2013.130710},
ISSN={0733-8716},
month={July},}

@ARTICLE{Joe,
author={C. Joe-Wong and S. Sen and S. Ha and M. Chiang},
journal={IEEE Journal on Selected Areas in Communications},
title={Optimized Day-Ahead Pricing for Smart Grids with Device-Specific Scheduling Flexibility},
year={2012},
volume={30},
number={6},
pages={1075-1085},
keywords={electric generators;electricity supply industry;power system economics;pricing;scheduling;smart power grids;control-feedback loop;device-specific scheduling flexibility;electricity generator;electricity provider;optimized day-ahead pricing;power grid;smart grids;time-dependent pricing;two-way communication;Delay;Electricity;Energy consumption;Generators;Optimization;Pricing;Sensitivity;Smart-Grid pricing;day-ahead pricing;demand response;patience index},
doi={10.1109/JSAC.2012.120706},
ISSN={0733-8716},
month={July},}

@book{Saadat,
  title={Power System Analysis},
  author={Saadat, H.},
  isbn={9780984543809},
  edition = {3rd}
  lccn={2010906755},
  url={https://books.google.es/books?id=s\_IbSQAACAAJ},
  year={2010},
  publisher={PSA Publishing}
}


@book{Saadat_old,
   author = {H. Saadat},
   title = {Power System Analysis},
   edition = {2nd}
   published = {McGraw-Hill}, 
   year = 2002 
}

